Frequency Response from Aggregated V2G Chargers With Uncertain EV Connections

Fast frequency response (FR) is highly effective at securing frequency dynamics after a generator outage in low inertia systems. Electric vehicles (EVs) equipped with vehicle to grid (V2G) chargers could offer an abundant source of FR in future. However, the uncertainty associated with V2G aggregation, driven by the uncertain number of connected EVs at the time of an outage, has not been fully understood and prevents its participation in the existing service provision framework. To tackle this limitation, this paper, for the first time, incorporates such uncertainty into system frequency dynamics, from which probabilistic nadir and steady state frequency requirements are enforced via a derived momeent-based distributionally-robust chance constraint. Field data from over 25,000 chargers is analysed to provide realistic parameters and connection forecasts to examine the value of FR from V2G chargers in annual operation of the the GB 2030 system. The case study demonstrates that uncertainty of EV connections can be effectively managed through the proposed scheduling framework, which results in annual savings of {\pounds}6,300 or 37.4 tCO2 per charger. The sensitivity of this value to renewable capacity and FR delays is explored, with V2G capacity shown to be a third as valuable as the same grid battery capacity.

==> Frequency Security Constraints/Freq_Sec_Cons.tex <==
%To ascertain the substantial system value of FR from aggregated EV fleets with V2G chargers, a pre-existing scheduling model is significantly enhanced to optimally co-ordinate charge and generation decisions in light of uncertain future EV connections. This section briefly introduces the advanced SUC model and the previously derived frequency security constraints \cite{Badesa2019,Teng2016}. To improve clarity decision variables are emboldened throughout.

\subsection{Stochastic Unit Commitment} \label{SUC Section}

The SUC model optimally schedules generator and storage actions to provide reserve, response (fast and slow), inertia and energy production under uncertain renewable output. User defined quantiles of the random variable of net demand (demand net of wind power) are used to construct a scenario tree. Reference \cite{Sturt2012} demonstrates that well chosen quantiles that branch only at the root node can discretize the continuous range of potential wind realisations in an accurate manner whilst yielding a highly tractable model. 

Each node has a complete set of decision variables, subject to standard generator and storage constraints including minimum stable generation, maximum (dis)charge, state of charge limits and the power balance constraint:
\begin{multline}
\label{power balance}
    \sum_g^G \boldsymbol{P_g}(n) + \sum_s^S \boldsymbol{P_s}(n) + \sum_i^I \boldsymbol{P^{EV}_i}(n) + P^w(n)- \boldsymbol{P^{wc}}(n)
    \\ + P^{sol}(n) - \boldsymbol{P^{solc}}(n) = P^d(n) - \boldsymbol{P^{LS}}(n)
\end{multline}
There are also inter timestep constraints between nodes to define states of charge, plant commitment times and minimum up/down times. An exhaustive constraint list can be found in Section III of \cite{Sturt2012}. The probability of reaching a given scenario (node) weights the cost function:
\begin{equation}
\sum_{n\epsilon N} \pi(n) \bigg( \sum_{g\epsilon G} \boldsymbol{C_g}(n) + \Delta \tau (n) (c^{LS} \boldsymbol{P^{LS}}(n)) \bigg)\label{Cost Function}
\end{equation}
A rolling planning approach is used to simulate annual system operation. Decisions that minimise the expected operating cost over the next 24h period are found. The decisions at the current root node are implemented and the system is rolled forwards by an hour, updating system states as well as wind and EV connectivity realisations. With this new information the scenario tree is updated and the process iterated.





\subsection{Frequency Security Constraints}\label{frequency security cons}
Each node in the scenario tree has a complete set of decision variables so the \textit{n} notation is dropped for clarity. System frequency evolution post generator loss can be accurately approximated by the single machine swing equation \cite{KundurBook}: 
\begin{equation}
\label{swng equation}
\frac{2 \boldsymbol{H}}{f_0} \frac{d \boldsymbol{\Delta f}}{d t} = \boldsymbol{R_1}(t) + \boldsymbol{R_2}(t) - \boldsymbol{PL_{max}}
\end{equation}
Equation (\ref{swng equation}) neglects load damping because the level in future systems dominated by power-electronics will be much reduced \cite{Chavez2014}. As in \cite{Chavez2014,Teng2016,Badesa2019, Badesa2020}, FR is modelled as a linear ramp. Detailed dynamic simulations carried out in Section III of \cite{Badesa2020} show that droop controls can be accurately and conservatively approximated by a ramp. More detailed dynamic models prohibit closed form solutions to (\ref{swng equation}), necessary in order to derive convex algebraic frequency security constraints.
\begin{equation}
\label{Unit ramp}
\boldsymbol{R_{k}}(t) = 
    \begin{cases} 
      \frac{\boldsymbol{R_{k}}}{T_{i}}\cdotp t & t \leq T_{k} \\
      \boldsymbol{R_{k}} & t > T_{k} \\
    \end{cases}
    \, k \in 1,2
\end{equation}
In this paper $T_1 < T_2$. The slower speed models governor controlled FR from thermal plants. The faster speed can come from power-electronic devices, distributed or otherwise:
\begin{equation}
\label{R1 composition}
\boldsymbol{R_1} = \boldsymbol{R^{ND}} + \boldsymbol{R^{EV}}
\end{equation}
\subsubsection{RoCoF Constraint}
%If including the response effect on RoCoF
%Relays require several frequency periods to accurately measure the frequency. Hence the RoCoF is a calculated as the average over some sampling period ($T_s$). The maximum RoCoF occurs in the sampling period immediately after generation loss. It must be limited in order to prevent the tripping of distributed generation via RoCoF-sensitive protection systems:
%\begin{equation}
%\label{RoCoF}
%|RoCoF| = \frac{|\boldsymbol{\Delta f}(T_p)|}{T_p} \leq |RoCoF_{max}| 
%\end{equation}
%Assuming $T_p < T_1$, an expression for $\Delta f(T_p)$ can be found by integrating (\ref{swng equation}) between 0 and $T_s$ \cite{omalley2021probabilistic}. Substituting this into (\ref{RoCoF}) results in a linear RoCoF constraint: 
%\begin{equation}
%\label{RoCoF.2}
% \frac{T_p}{2T_1} \cdotp R_1 + \frac{T_p}{2T_2} \cdotp R_2 + \frac{2 |RoCoF_{max}|}{f_0} \cdotp H \geq PL_{max}
%\end{equation}

%Not including response impact on RoCoF
The maximum RoCoF occurs at the moment of $PL_{max}$ outage. At this time no response has been delivered so it is limited by inertia alone, necessary to prevent RoCoF-sensitive protection systems from disconnecting distributed generation and exacerbating the deficit. Setting $t=0$ in (\ref{swng equation}) results in:
\begin{equation}
\label{RoCoF.2}
  \frac{2 |RoCoF_{max}|}{f_0} \cdotp \boldsymbol{H} \geq \boldsymbol{PL_{max}}
\end{equation}
\subsubsection{Nadir Constraint}
To insure that the nadir occurs before $T_2$, the sum of FR must be greater than the largest loss:
\begin{equation}
\label{steady state}
\boldsymbol{PL_{max}} \leq \boldsymbol{R_1} + \boldsymbol{R_2}
\end{equation}
Here it is assumed that the nadir occurs after $T_1$ ($\approx 1$s) as the extremely low inertia required to breach the frequency limit $\Delta f_{max}$ ($\approx -0.8$Hz) would violate the RoCoF constraint (\ref{RoCoF.2}) for realistic power system parameters. The frequency nadir occurs at the instant of zero RoCoF. According to (\ref{swng equation}) this is:
\begin{equation}
\label{Nadir time}
\boldsymbol{t^*} = \frac{(\boldsymbol{PL_{max}}-\boldsymbol{R_1})\cdotp T_2}{\boldsymbol{R_2}}
\end{equation}
It is shown in \cite{Badesa2019} that by integrating (\ref{swng equation}) and then substituting in (\ref{Nadir time}), the nadir constraint can be formed as a convex rotated SOC:
\begin{equation}
\label{Nadir Constraint}
\bigg(  \underbrace{ \frac{\boldsymbol{H}}{f_0}-\frac{\boldsymbol{R_1} \cdotp T_1}{4 \Delta f_{max}} }_{= \ \boldsymbol{z}} \bigg)\hspace{-0.1cm}\underbrace{ \frac{\boldsymbol{R_2}}{T_2} }_{= \ \boldsymbol{x}} \hspace{-0.1cm} \geq \hspace{-0.1cm} \bigg(\underbrace{\frac{\boldsymbol{PL_{max}} - \boldsymbol{R_1} }{2 \sqrt{\Delta f_{max}}}}_{= \ \boldsymbol{y}}  \bigg)^2
\end{equation}

Finally, the power injection from aggregated chargers may be delayed due to communication or frequency measurement lag. An additional term in the Nadir constraint can account for this \cite{Badesa2020}:
\begin{equation}
\label{Delay definition}
\boldsymbol{z} = \frac{\boldsymbol{H}}{f_0}-\frac{(\boldsymbol{R^{ND}} + \boldsymbol{R^{EV}}) \cdotp T_1 }{4 \Delta f_{max}} - \frac{\boldsymbol{R^{EV}} \cdotp 2 T_{del} }{4 \Delta f_{max}}
\end{equation}
